LLaVA-Grounding: Grounded Visual Chat with Large Multimodal Models

With the recent significant advancements in large multi-modal models (LMMs), the importance of their grounding capability in visual chat is increasingly recognized. Despite recent efforts to enable LMMs to support grounding, their capabilities for grounding and chat are usually separate, and their chat performance drops dramatically when asked to ground. The problem is the lack of a dataset for grounded visual chat (GVC). Existing grounding datasets only contain short captions. To address this issue, we have created GVC data that allows for the combination of grounding and chat capabilities. To better evaluate the GVC capabilities, we have introduced a benchmark called Grounding-Bench. Additionally, we have proposed a model design that can support GVC and various types of visual prompts by connecting segmentation models with language models. Experimental results demonstrate that our model outperforms other LMMs on Grounding-Bench. Furthermore, our model achieves competitive performance on classic grounding benchmarks like RefCOCO/+/g and Flickr30K Entities. Our code will be released at https://github.com/UX-Decoder/LLaVA-Grounding .

==> images/intro_fig1.tex <==
% \begin{figure}[tbh]
% % \centering  
% % \vspace{-0mm}
% \includegraphics[width=0.5\textwidth]{images/src/Intro.pdf}
% % \vspace{-2mm}
% \caption{Comparisons.}
% \label{fig:Comparisons}  
% % \vspace{-3mm}
% % \hao{chat, grounding, legend in image,model size}
% \end{figure}



\begin{figure}[t]
\begin{minipage}{1.0\linewidth}
  \centering
  % 图片
  \includegraphics[width=1.0\linewidth]{images/src/Intro.pdf}
\end{minipage}
\begin{minipage}{1.0\linewidth}
  % 表格
  \footnotesize
    % \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{lllll|llll}
    \toprule
             & \multicolumn{4}{c|}{input} & \multicolumn{4}{c}{output} \\
             & text & click & box & mark & text  & box & mask & mark \\
             \midrule
    LLaVA    &   \checkmark   &       &     &      &       \checkmark&       &     &      \\
    MiniGPT4 &  \checkmark    &       &     &      &       \checkmark&       & &      \\
    GPT4ROI  &  \checkmark    &       &  \checkmark   &      &       \checkmark&       &     &      \\
    Shikra   &    \checkmark  &       &     &      &       \checkmark&       &     &      \\
    Ferret   &   \checkmark   &    \checkmark   &     &      &       \checkmark&     \checkmark  &     &      \\
    miniGPTv2   &  \checkmark    &       &     &      &       \checkmark&  \checkmark   &     &      \\
    LLaVA1.5   &  \checkmark    &       &     &      &       \checkmark&  \checkmark   &     &      \\
    CogVLM   &  \checkmark    &       &     &      &       \checkmark&  \checkmark   &     &      \\
    Ours     &    \checkmark  &    \checkmark   &   \checkmark  &   \checkmark   &  \checkmark     &    \checkmark   &   \checkmark  &     \checkmark  \\
    \bottomrule
    \end{tabular}
    % }
  \caption{Comparison \hao{Language may change to visual chat. update the number of shikra} \jianwei{add cite to these works}}
  \label{fig:table-and-figure}
\end{minipage}
\end{figure}

==> images/vis_supp_vp.tex <==
\begin{figure*}[t!]
\centering  
\vspace{-0mm}
\includegraphics[width=0.99\textwidth]{images/src/vis_visual_prompt.pdf} \\
% \vspace{-2mm}
\caption{Comparison of our method with Shikra in visual prompts. In the left block, the red star is user's click and the highlight region in response is the predicted mask from the prompt encoder. In the right block, the red box is drawn by the user. }
\label{fig:visualization supp vp}  
% \caption{}
  % \vspace{-5mm}
\end{figure*}

==> images/visualization.tex <==
\begin{figure*}[h!]
\centering  
\vspace{-0mm}
\includegraphics[width=\textwidth]{images/src/visualization_v1.pdf} \\
\vspace{-2mm}
\caption{\footnotesize Visualization of our model. (1) Grounded detail description; (2) Visual prompts; (3) Potentially reduce hallucination; (4) Mark prompts for grounding.}
% \hao{finegrained dog class}
\label{fig:visualization}  
% \caption{}
  % \vspace{-5mm}
\end{figure*}

==> tables/algorithm_bench.tex <==
\begin{figure}[t]
  % Shared Initialization
  % \begin{minipage}{\textwidth}
        % content = '''
        % generate image captions with grounded entities and attributes with following information: \n
        % pseudo image description: <{}>, \n
        % ground truth image captions: <{}>, \n
        % ground truth bounding boxes ([x0,y0,w,h]: (x0,y0) is the top-left corner, (w,h) is box size), category_info, and entity_id: <{}>, \n
        % entity_proposal: <{}>, \n
        % an example output format would be: "[entity_id]<A woman> sitting next to [entity_id]<a handsome man>, with their hands holding together under [entity_id]<the blue sky>.", where [entity_id] and <xxx> are associated with the ground truth bounding boxes. \n
        % entity_id is the real id number in the ground truth bounding boxes. \n
        % generated caption constraints:
        % (1) rely more to ground truth image captions, rely less on image description. 
        % (2) the entity in the generated caption should be in entity_proposal.
        % (3) the generated entity nouns could rely on object_descriptions in ground truth image captions.
        % (4) for [entity_id] and <xxx>, the content in <xxx> is better to include the adj description.
        % (5) the generation caption should have less hallucinate description in image description. \n
        % '''.format(_llava_caption, _coco_caption, _coco_panoptic, _coco_entity)
    
  \begin{algorithm}[H]
      \caption{Pseudo code for \benchname{} Evaluation}
      \label{alg:shared_initialization}
      \scriptsize
      \Comment{Inputs: Grounded response $(T,\mathbf{b})$; GT response and boxes $(\hat{T},\hat{\mathbf{b}})$.}
      \Comment{Outputs: Chat scores ($\mathbf{S}$); Grounded response scores ($P$, $R$, $F_1$).}
      \Comment{Functions: GPT\_chat\_eval(), match\_gt\_box(), construct\_gd\_response(), GPT\_gd\_eval(), calc\_scores().}
          % \Comment{Variables:~Learnable Queries($Q_h$); Attention Masks between $Q$ and $P$(qpm)}         \Comment{Functions:~Img\_Encoder(),Text\_Encoder(),Visual\_Sampler(),feature\_attn(),prompt\_attn(),output();}
  \Function{GroundingBenchEval($T,\mathbf{b}$,$\hat{T},\hat{\mathbf{b}}$)}{
     \var{$\mathbf{S}$ = GPT\_chat\_eval($T$,$\hat{T}$)} \Comment{Request GPT-4 to score $T$}
     % \var{$TP_{pred}$=0,$TP_{gt}$=0}\Comment{initialize}
     \var{$N_{gt}$=len($\hat{\mathbf{b}}$), $N_{pred}$=len($\mathbf{b}$)} 
     
     \var{$\textbf{b}_{matched}$ = []}
     
     \For{$b$ in $\mathbf{b}$}{
        \var{gt\_box, iou = match\_gt\_box($b$,$\hat{\mathbf{b}}$)} 
        
        \If{$iou\geq 0.5$}{
            \var{$\textbf{b}_{matched}$=$\textbf{b}_{matched}$+gt\_box}
        }
        
     } 
     % \tianhe{we may add some annotations in pseudo code}
     \var{$T_{eval}$ = construct\_gd\_response($T$,$\textbf{b}_{matched}$)}\Comment{Insert matched gt boxes into the response to form responses of Context type 3 in Table~\ref{tab:full_example_car_bbox}}

     % \Comment{$T_{eval}$: }
     
    \var{$TP_{pred}$,$TP_{gt}$ = GPT\_gd\_eval($T_{eval}$)} \Comment{GPT help evaluate semantic matching}
    
    \var{$P$, $R$, $F_1$ = calc\_scores($TP_{pred}$,$TP_{gt}$,$N_{gt}$)} \Comment{Calculate grounded response scores}

    \var{output = $\mathbf{S}$, $P$, $R$, $F_1$}
    
    \Return{output}
    
     % for b in $\mathbf{b}$:
     %    iou=max(IoU(b,$\hat{\mathbf{b}}$))
     %    if iou<0
     % \var{Content = \textcolor{gray}{```}generate image captions with grounded} 
     % \var{entities and attributes with following: \; \; \;}
     % \var{\textcolor{blue}{pseudo image description}:~<\textcolor{red}{\{\}}>, \; \; \; \; \; \; \; \;  \; \;  \; \;}
     % \var{\textcolor{blue}{ground truth image captions}:~<\textcolor{red}{\{\}}>, \; \; \; \; \; \; \; \;  \; \;  \; \; }
     % \var{ground truth bounding boxes (x0,y0,w,h): (x0,y0) is the top-left corner, (w,h) is box size), \textcolor{blue}{categor\_info, and entity\_id}:~<\textcolor{red}{\{\}}>, \; \; \; \; \; \; \; \;  \; \;}
     % \var{\textcolor{blue}{entity\_proposal}: <\textcolor{red}{\{\}}>, \; \; \; \; \; \; \; \;  \; \; \; \; \;  \; \; \;  \; \;}
     % \var{an example output format would be: "(entity\_id)<A woman> sitting next to (entity\_id)<a handsome man>, with their hands holding together under (entity\_id)<the blue sky>.", where \textbf{(entity\_id)~and~<xxx>~are associated with the ground truth bounding boxes.} \textbf{entity\_id is the real id number in the ground truth bounding boxes.} generated caption constraints:~1.~xxx; 2.~xxx; \textcolor{gray}{'''}.\textcolor{red}{format}(llava\_cap, coco\_cap, coco\_pano, lvis\_inst))
     % };
     
     % \var{output = GPT4(content)}
     }
  % \Function{SEEM\_Decoder($F_v$,$Q_o$,$Q_t$,$Q_v$,$P_v$,$P_t$,$P_m$)}{
  %   \var{
  %   $Q_o$,$Q_t$,$Q_v$ = feature\_attn($F_v$,$Q_o$,$Q_t$,$Q_v$)}; \Comment{Cross attend queries with image features.}
  %   \var{
  %     $Q_o$,$Q_t$,$Q_v$ = prompt\_attn(qpm,$Q_o$,$Q_t$,$Q_v$,$P_v$,$P_t$,$P_m$)}; \Comment{Self attend queries and prompts.}

  %   \var{
  %     $O_m$,$O_c$,$P_m$ = output($F_v$,$Q_o$,$Q_t$,$Q_v$)}; \Comment{Compute mask and class outputs.}
  % }
  % \Function{forward(img,pm,nm,txt)}{
  %    \var{$F_v$,$Q_o$,$Q_t$,$Q_v$,$P_v$,$P_t$ = init(); $P_m$ = None}; \Comment{Initialize variables.}
  %    \For{$i$ in range(max\_iter)}{
  %   \var{$O_m$,$O_c$,$P_m$ = SEEM\_Decoder($F_v$,$Q_o$,$Q_t$,$Q_v$,$P_v$,$P_t$,$P_m$)}
  %    }
  % }
  \end{algorithm}
  \label{algo}
  % \end{minipage}
\vspace{-25pt}
\end{figure}

==> tables/our_bench.tex <==
\begin{table*}[t!]
\centering
\scalebox{0.7}{
\begin{tabular}{l|c|c|ccc|cccc|c}
\toprule
 &  Prompt &\#Vision& \multicolumn{3}{c|}{Grounded Response Scores}& \multicolumn{4}{c|}{Chat Scores}&Phrase\\

 % & &\toprule\multicolumn{3}{c}{Grounding Caption}& \multicolumn{4}{c}{Language}&\\

Model&     type& params(B)&Recall&Precision&$F_1$&Detail desc.& Conv.& Reasoning & \textbf{All}  &\multicolumn{1}{c}{grounding}\\
\midrule
% LLaVA& - &0.30& $--|--$& $--|--$& $--|--$& 69.1 & 82.0 & 92.6 & 81.2 & -\\
LLaVA~\cite{liu2023visual}& - &0.30&- &- &-& 69.1 & 82.0 & 92.6 & 81.2 & -\\
Shikra~\cite{chen2023shikra}    & GVC &0.30& $26.9|22.8$& $55.6|42.5$& $36.2|29.7$& 64.7 & 75.4 & 86.4 & 75.5 & 64.29\\
Shikra    & GD       &0.30& $30.6|21.7$& $47.9|44.3$& $37.3|30.9$& 41.8 & -    & -    & -    & - \\
miniGPT v2~\cite{chen2023minigptv2}& GVC &0.30& $29.2|22.6$& $43.9|36.4$ & $35.1|27.9$ & 48.0& 51.0& 38.7& 45.8& -\\
CogVLM~\cite{wang2023cogvlm}    & GVC &10.0& $32.7|15.2$& $72.5|67.6$& $45.1|33.2$ & 35.8& 47.8& 22.2& 34.9& - \\
CogVLM    & GD       &10.0& $32.8|23.0$& $74.4|58.6$& $45.5|33.0$& 36.4& -& -& -& - \\
% Kosmos2   &         &&&&& & & &\\

GPT4-V$^*~\cite{gpt4v}$& -       &-& $55.1|--$& $73.5|--$& $63.2|--$& 67.3    & 104.3    & 108.4    & 93.3& \\
\midrule
\rowcolor{gray!15} \shortname{} (Ours)      & GVC & 0.35&      $46.8|29.3$&   $54.2|54.4$&   $50.2|38.1$& 67.2  & 78.7  & 91.1  &  79.3 &81.6   \\
\bottomrule
\end{tabular}
}

% GPT4v language
% llava-1.5
\vspace{-5pt}
\caption{\footnotesize 
\hao{bubogpt} 
% \hao{13B+swinl}
% \hao{compare with other methods (grounding, chat)}
\hao{click use point,appendix visual prompt two images,re-draw visulizations}
\hao{re-test 1k for all methods}
\hao{demo}  
For the chat scores, we follow LLaVA to prompt GPT-4 with the answers from our model outputs and the answers by GPT-4 (text-only), and let it compare between both responses and give a rating with an explanation.
Where ``GVC'' denotes the grounded visual chat prompt in our \benchname{}. ``GD" denotes specialized grounded description (GD) prompt recommended by the corresponding method. $^*$ denote we use SoM~\cite{yang2023setofmark} to prompt GPT4-V.  \chunyl{Report GPT-V results without SoM. This help sell the proposed work}\hao{GPT-V cannot do ground visual chat, do we need to remove gpt4-v row?} 
}
% \hao{update phrase grounding for shikra}}
% \hao{ego-4d,菜谱，修自行车，手机端zoomin zoomout,直播带货双击}
\label{tab: our bench}
\vspace{-0.4cm}
\end{table*}
